Bridging the Language Gaps in Large Language Models with Inference-Time Cross-Lingual Intervention

Large Language Models (LLMs) have shown remarkable capabilities in natural language processing but exhibit significant performance gaps among different languages. Most existing approaches to address these disparities rely on pretraining or fine-tuning, which are resource-intensive. To overcome these limitations without incurring significant costs, we propose Inference-Time Cross-Lingual Intervention (INCLINE), a novel framework that enhances LLM performance on low-performing (source) languages by aligning their internal representations with those of high-performing (target) languages during inference. INCLINE initially learns alignment matrices using parallel sentences from source and target languages through a Least-Squares optimization, and then applies these matrices during inference to transform the low-performing language representations toward the high-performing language space. Extensive experiments on nine benchmarks with five LLMs demonstrate that INCLINE significantly improves performance across diverse tasks and languages, compared to recent strong baselines. Our analysis demonstrates that INCLINE is highly cost-effective and applicable to a wide range of applications. In addition, we release the code to foster research along this line: https://github.com/weixuan-wang123/INCLINE.

==> _analysis.tex <==


\section{Analysis}
\label{sec:analysis}

\subsection{Correct Prediction Overlap}
\label{sec:analysis_cpo}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.65]{figures/xltr-acc.pdf}
    \caption{Correct prediction overlap (CPO) and accuracy from English to non-English on \xcopa for models with \ours.}
    \label{fig:cpo}
\end{figure}

We analyzed the Correct Prediction Overlap (CPO) between English and non-English languages using the \xcopa test set. CPO represents the percentage of questions that are correctly answered in both English and a non-English language. The overlap ratio and accuracy are presented in \autoref{fig:cpo}. The results show that \ours significantly improves both accuracy and the performance overlap ratio. Notably, the overlap for Vietnamese increased from a baseline of 0.77 to 0.94, indicating that \ours corrected previously incorrect answers for Vietnamese questions. This finding further supports \ours's ability to align non-English representations with English representations.



% \subsection{Visualization of Latent Space}


% Experimental results have demonstrated the benefits of cross-lingual intervention. For a more intuitive depiction of the English and non-English spaces in the LLMs, we reduce the hidden states of English and Portuguese sentences to 2 dimensions using t-SNE and visualize their kernel density estimate distribution in \autoref{fig:projection-ori}. The visualization reveals a clear separation between English and Portuguese samples, highlighting a representation gap between multilingual inputs. However, post-intervention with \ours, this cross-lingual gap is significantly reduced, with representations showing substantial overlap in \autoref{fig:projection-incline}. It means that \ours effectively enhances the alignment of model representations. Further visualization details are available in Appendix~\ref{appendix-visualize}.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{figures/acc-time.pdf}
    \caption{Effects of the amount of training data for projection vector with evaluating on \xstorycloze in Swahili for \ours with \bloomz.}
    \label{fig:acc-time}
\end{figure}

\subsection{Computing Cost}
\label{sec:analysis_cost}

To demonstrate the trade-off between computational cost and accuracy, we measured the time consumed in training the projection matrix and evaluated \ours on the \xstorycloze task in Swahili. As illustrated in \autoref{fig:acc-time}, increasing the amount of training data does not necessarily enhance accuracy, although training time is directly proportional to the number of training samples. With just 500 samples, our training process took only 172 seconds, showcasing its low cost.

Since the single intervention occurs only at the last token, the time complexity of our method during inference is $O(1)$. The additional time consumed is only 12\% more than the original processing time (0.80 seconds per item with our method vs. 0.71 seconds per item without it, as shown in \autoref{tab:infer-time} in Appendix \ref{sec:appendix-infertime}).

==> _dicussion.tex <==
\section{Discussion}
\label{sec:discussion}

% \subsection{Multilingual Prompt Template}
% \label{sec:multilingual-prompt}

% \input{tables/multilingual_prompt}

% To better understand \ours and reinforce our interpretations, we carried out ablation studies that assess the performance differences between using English and non-English prompt templates on the \xcopa dataset, as shown in \autoref{tab:non-english prompt}. \ours achieves greater improvements with the English template than with the multilingual template, with increases of up to +2.58 versus +2.07 in average accuracy. The baseline performance with multilingual template is lower than that with English template, indicating the different comprehension capabilities of multilingual prompt templates. \ours depends on the representations of the last token, which contains all information processed by the LLMs. Consequently, any misunderstandings in the input persist even after being projected into the English space. Therefore, the performance with multilingual templates and intervention is generally lower than with the English template across languages.

% \subsection{Effective across Multiple LLMs}
% \label{sec:morellms}
\input{tables/llms}
\paragraph{\ours consistently enhances performance across multiple LLMs.} To demonstrate the effectiveness of \ours across different LLMs, we apply \ours to five other well-performing models: \bloomz, \llamathree, \llama, \mistral, and \falcon on the \xstorycloze task. As shown in \autoref{tab:otherllms}, \ours consistently enhances performance compared to the \baseline. Specifically, we observe increases of +4.96 points for \bloomz, +5.40 points for \llamathree, +7.03 points for \llama, +8.64 points for \mistral, and +2.74 points for \falcon. These results confirm \ours's effectiveness across various LLMs.


% \subsection{Effect of Few Shots}

% \input{tables/fewshots}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{figures/few-shots.pdf}
    \caption{The averaged EM score for \mzsre dataset with \ours based on the zero-shot setting and few-shot settings given by \bloomz.}
    \label{fig:scale}
\end{figure}
\paragraph{Less improvement in few-shot settings since examples already guide learning.}According to \citet{mzsre}, in-context learning (ICL) can improve the performance of an LLM under the guidance of few-shot examples in the cross-lingual Knowledge Editing task. We expanded this exploration to assess the impact of few-shot examples on \ours on the \mzsre dataset. As shown in \autoref{fig:scale}, \ours performs well in a 4-shot setting, showing an increase in the average Exact Match (EM) score by +1.02. When compared to the 0-shot setting, this improvement is smaller (+1.02 vs. +3.26). This suggests that few-shot examples already provide a strong learning signal (to \baseline), somewhat overshadowing the additional benefits derived from hidden states semantic alignment.


% \subsection{Scaling the Size of LLMs}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{figures/scale.pdf}
    \caption{Averaged EM score on \textsc{BLOOMZ} series on \mzsre dataset. The improvement indicated on the second y-axis represents the percentage improvement relative to the baseline.}
    \label{fig:scale}
\end{figure}
\paragraph{Larger LLMs benefit more from \ours.} Previous work by \citet{mzsre} demonstrated a scaling relationship between the size of the backbone model and its performance. Building on this, we evaluate the impact of different model sizes within the \textsc{BLOOMZ} series on the \mzsre dataset. The EM scores, presented in the stacked column chart, and the improvement percentage depicted in the line chart in \autoref{fig:scale}, show that the relative performance gain of \ours over the baseline increases with the size of the backbone model. For instance, larger models in the \textsc{BLOOMZ} series show more significant improvements when \ours is applied. This suggests that larger multilingual LLMs align more effectively with the representations learned by \ours.

% \subsection{Projection to Non-English}

% \input{tables/fr}

% We have shown that translating to English improves when projecting representations from non-English to English. We conducted an ablation study to explore the effects of projecting into another language, specifically translating into French, and assessed \ours's performance. As shown in \autoref{tab:xx2fr}, \ours also enhances the performance of translating to non-English languages, evidenced by an average increase in BLEU score of +0.815. This further demonstrates that \ours can effectively align representations across different languages.


% \subsection{Domain of Training Data for Projection}
\input{tables/ood}
\paragraph{In-domain data leads to better improvements with \ours.} To evaluate the impact of data domain on \ours, we train the projection matrix using in-domain data from the Flores development set (\oursind) and out-of-domain data from the News Commentary dataset (\oursood). As shown in \autoref{tab:domain}, the in-domain intervention (\oursind) outperformed the out-of-domain intervention (\oursood), achieving an average BLEU score increase of +2.75 points. This indicates that careful selection of training data is crucial when implementing \ours, as it helps minimize the negative effects of domain shifts on language projection vector training.

==> _experiments.tex <==



\section{Experimental Results}
\label{sec:results}

In this section, we demonstrate the experimental results, involving a comprehensive range of tasks, from multiple-choice to open-ended generation tasks. Moreover, we analyse the influence of intervened components, and the influence of the direction of intervention.


% \input{tables/main}

As \bloomz is fine-tuned on training dataset XP3, we split the involved languages into two groups according to if the traning data of this language is included in the datasets: seen languages (ar, es, fr, hi, id, pt, sw, ta, vi, zh), unseen languages (de, el, et, it, ja, nl, ru, th, tr). The results of multiple-choice tasks (\xcopa, \xstorycloze, \xwinograd, \xcsqa, \xnli) and the results of open-ended generation tasks (\mzsre, \flores, \wmt, \mgsm) are shown in \autoref{tab:main-mc} and \autoref{tab:main-gen}, respectively.


% \paragraph{\ours significantly improves multiple-choice task performance.}
% The experimental results in \autoref{tab:main-mc} highlight the importance of effective cross-lingual representation alignment in multilingual NLP tasks. 
% The significant drop of \baseline from seen to unseen languages indicates the model's limited ability to generalize to unseen languages, reflecting its reliance on pre-existing language representations. 
% While translation methods (\mtgoogle, \mtllm) provide a straightforward approach to multilingual tasks, their effectiveness is highly dependent on translation quality and the linguistic coverage of the model. However, this approach may not always be practical.
% \sft demonstrates that task-specific fine-tuning can substantially improve performance. However, it demands considerable computational resources and may not generalize across languages.
% While \iti and \caa provide modest improvements over the baseline without retraining the entire model, the improvements are limited, suggesting these methods may not effectively address the underlying representation misalignments across languages.


\paragraph{\ours significantly improves multiple-choice task performance.}
The experimental results in \autoref{tab:main-mc} demonstrate that while methods like \sft and \mtgoogle can achieve high performance, they come with significant costs or dependencies. Activation adjustment methods (\iti and \caa) provide modest improvements but may not capture the necessary semantic complexities. \ours presents great advantages by effectively enhancing multilingual representation alignment at inference time without extensive retraining or external dependencies, thereby improving the multilingual performance in a more efficient way. \ours significantly improve the performance across languages with increasing the averaged accuracy by up to +4.96, and reaching up +4.20 and +9.46 for the seen and unseen languages, respectively. The enhancement on the unseen languages proves the effectiveness of \ours in aligning the semantic representation between languages.


\paragraph{\ours significantly improves open-ended generation task performance.}
The experimental results also highlight the effectiveness of \ours in open-ended generation tasks, achieving an increase of up to +5.09 on the \flores task, as shown in \autoref{tab:main-mc}. For the \mgsm task, which involves the reasoning abilities of LLMs, \ours enhances the model's reasoning capability in English by aligning semantic representations from non-English inputs to English. The consistent improvements across various tasks and languages suggest that \ours is a practical and efficient solution for multilingual applications seeking a balance between performance and resource expenditure. Detailed results for each language and task are provided in \autoref{tab:overall} (see Appendix \ref{sec:appendix-detail}).


Compared to the \iti and \caa, \ours demonstrates significant improvements, primarily stemming from two reasons. First, unlike \iti and \caa which intervenes in certain attention heads or hidden states in one layer to shift towards English representations, \ours modifies the overall representations, thereby enhancing the projection into the English space more comprehensively. Additionally, simple adjustments with a static intervention is inadequate for learning the projection from non-English to English; instead, \ours employs the Least-Squares to fit the projection, ensuring better alignment between cross-lingual semantic representations. 

\input{latex/tables/configuration}

\paragraph{Intervention on hidden states enhances performance the most.}
To further evaluate the effectiveness of \ours, we applied it to various components of LLMs, including the outputs of attention heads (\oursattn), the outputs of activation functions in feed-forward networks (FFNs) (\oursact), the outputs of FFN blocks (\oursffn), and the embeddings (\oursemb). The results in \autoref{tab:config} indicate that intervening on the hidden states (\ourshidden) yields the most significant improvements across multilingual tasks. This suggests that the hidden states capture comprehensive semantic information crucial for cross-lingual alignment. While \oursattn, \oursact, \oursffn, and \oursemb also enhance performance, the magnitude of their gains varies. Notably, all intervention methods outperform the baseline, underscoring the effectiveness of aligning internal representations to achieve semantic alignment between non-English and English inputs.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.7]{latex/figures/parameter_2langs.pdf}
    \caption{The accuracy changed with hyperparameter $\alpha$ on the \xstorycloze task with \bloomz.}
    \label{fig:parameter}
\end{figure}


\paragraph{The direction of intervention relates to language similarity.}
In \autoref{fig:parameter}, we conducted a grid search to find the optimal $\alpha$ values for Spanish and Chinese, examining their effects on the model's accuracy on the \xstorycloze dataset. Given that Spanish and English belong to the same language family, whereas Chinese belongs to a different family, we observed that the optimal $\alpha$ values for these two languages are opposite: positive for Spanish and negative for Chinese. The negative optimal value for Chinese indicates that the direction of semantic representations between English and Chinese is opposite, highlighting the influence of language similarity on the intervention. Detailed results for each language are provided in \autoref{fig:parameter-alllangs} (see \autoref{sec:appendix-direction}).





% As shown in \autoref{tab:main-mc} and \autoref{tab:main-gen}, \textbf{\ours} achieves SOTA results in both open-ended generation and multiple-choice tasks (\xwinograd), yielding maximum average performance improvements of +3.50 and +4.95 over the baseline, respectively. Unlike methods that rely on hard replacement by translating queries into English or \sft techniques, \ours directly enhance the alignment of multilingual representations during decoding without requiring additional tools or models, thereby improving the multilingual performance in a more efficient way.



% For the multi-choice tasks, \mtgoogle enhances performance across almost all languages and attains the highest average accuracy on the \xcopa, \xcsqa, and \xnli tasks. But \mtllm has the worst performance, indicating the poor translation quality of the LLM. The lower accuracy of \sft compared to the baseline highlights the difficulties in automatically transferring skills learned in English to other languages, which varies across tasks. Compared to the \iti, \ours demonstrates significant improvements, primarily stemming from two reasons. First, unlike \iti which intervenes in certain attention heads to shift towards English representations, \ours modifies the overall representations, thereby enhancing the projection into the English space more comprehensively. Additionally, simple adjustments with a linear classifier is inadequate for learning the projection from non-English to English; instead, \ours employs the Least-Squares to fit the projection, ensuring better alignment between cross-lingual representations. 

% For the open-ended generation tasks \mzsre and Flores, which produce English output, \ours enhances the alignment of sentence-level semantic within the internal representations, achieving a maximum improvement of +3.26 in average performance. For the \mgsm task, which generates non-English output, the improvement +3.5 further demonstrates the effectiveness of \ours in aligning semantics without affecting the output language. This further demonstrates that by combining non-English representations and projected representations, the intervention can maintain the linguistic features of the original language while aligning with English semantics.

% \textbf{Generalizability across tasks and languages} \ours significantly enhances multilingual performance across multiple languages and tasks compared to the baseline, with improvements reaching up to +9.46 (\xstorycloze-ru). Moreover, \ours outperforms \mtgoogle by substantial margins in certain languages (e.g., up to +11.2 for \xcopa in Tamil), indicating that aligning internal representations can ensure semantic alignment between non-English and English. The degree of improvement varies among languages; for example, the highest and lowest increases in the \xstorycloze task are +9.46 (ru) and +1.66 (id), respectively. Furthermore, the performance enhancements achieved through multilingual intervention is task-related, with gains for Chinese inputs across eight tasks ranging from +0.84 (\flores) to +5.11 (\mzsre). Despite its sensitivity to language settings and task variations, \ours consistently improves performances compared to baselines. Its strong generalization across diverse tasks and languages is primarily stems from the projection weights being trained on out-of-domain datasets, which helps maintain their semantic robustness.%which preserve their semantic integrity and generative capabilities.


% \subsection{Effect of Intervention Position}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[scale=0.5]{figures/radar.png}
%     \caption{The comparison of intervention in the hidden states (\ourshidden), the outputs of the attention layer (\oursattn), the activation function (\oursact), and the FFN block (\oursffn).}
%     \label{fig:radar}
% \end{figure*}



% We present the results of multilingual intervention in the hidden states, the outputs of the attention layer, the activation function, and the FFN block in \autoref{fig:radar}, respectively. \ours effectively aligns with English regardless of the specific position targeted for intervention, as evidenced by nearly all intervention results surpassing the baseline (indicated by the blue dot in \autoref{fig:radar}). Overall, interventions in the hidden states outperform interventions in other internal representations, based on average scores across all tasks and languages. However, the effectiveness of intervening in different representations varies by language and task. For instance, on the \xnli dataset, interventions in the hidden states yield the highest scores for Arabic, German, Greek, Hindi, and Chinese. In contrast, for Spanish, French, Swahili, Thai, and Vietnamese, the best results are obtained through interventions in the output of the attention layer. Detailed results for each type of intervention are presented in \autoref{tab:detail} in Appendix~\ref{app-detail}.



% \subsection{Patching Representation}
% \input{tables/patching}


% The target of \ours is to align the representation of non-English to English's representation. Hence, the ceiling of alignment is patching the representation of English inputs to the representation of corresponding non-English input. We patch the hidden states and the output of attention layer at the last token from English to non-English during decoding (wrt. patch-hidden and patch-attn). We present partial results in \autoref{tab:patch} and comprehensive results in \autoref{tab:patch-overall} in Appendix~\ref{appendix-patch}. 

% Patching hidden states achieves the same performance across languages with the results of English inputs for the \xcopa task, as the LLM only needs to output one token based on the last token's representations in multiple-choice tasks. However, patching the representations of attention layer generally reduces performance, except in the \mgsm task, due to the transformer’s residual connection preventing non-English representations from aligning closely with English ones. For open-ended generation tasks, the improvement from patching hidden states is slight. Furthermore, \ours outperforms the patching by up to +5.6 for \mgsm-zh, demonstrating its effectiveness in aligning multilingual representations. Additionally, \ours overcomes the limitations of relying on parallel test sets, which is a necessity for patching methods.



% \subsection{Direction of Projection}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[scale=0.65]{figures/parameter.pdf}
%     \caption{The accuracy changed with hyperparameter $\alpha$ on the \xstorycloze task.}
%     \label{fig:parameter}
% \end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.7]{latex/figures/parameter_2langs.pdf}
%     \caption{The accuracy changed with hyperparameter $\alpha$ on the \xstorycloze task with \bloomz.}
%     \label{fig:parameter}
% \end{figure}


% In \autoref{fig:parameter}, we conducted a grid search for the optimal $\alpha$ for each language to examine its effect on the model's accuracy on the \xstorycloze dataset. We observed that the optimal values for the intervention strength $\alpha$ differ across languages. A positive $\alpha$ value indicates that the projection direction from non-English to English, trained on the out-of-domain dataset, aligns with the direction required for the downstream test set. Conversely, a negative value indicates the opposite direction. Utilizing a small in-domain validation dataset to determine the best hyperparameter values is a practical approach.



==> _settings.tex <==
\section{Experiments}
\label{sec:settings}

We present our experimental task (\autoref{sec:setting-tasks}), baselines (\autoref{sec:setting-baseline}), and configurations (\autoref{sec:setting-configuration}) in this section.

\subsection{Tasks}
\label{sec:setting-tasks}

We apply \ours to multilingual LLMs to eight NLP tasks with aligning from non-English to English: multiple-choice tasks: \xcopa~\citep{xcopa}, \xstorycloze~\citep{xstorycloze}, \xwinograd~\citep{xstorycloze},  \xcsqa~\citep{xcsqa}, \xnli~\citep{xnli}; open-ended generation tasks: \mzsre~\citep{mzsre}, \flores~\citep{flores}, \mgsm~\citep{mgsm}. We include datasets that are diverse in terms of output format, tasks, and domains in \autoref{tab:dataset} (Appendix~\ref{sec:appendix-dataset}). The involved 20 languages includes English (en), Arabic (ar), German (de), Greek (el), Spanish (es), Estonian (et), French (fr), Hindi (hi), Indonesian (id), Italian (it), Japanese (ja), Dutch (nl), Portuguese (pt), Russian (ru), Swahili (sw), Tamil (ta), Thai (th), Turkish (tr), Vietnamese (vi), Chinese (zh). 

\input{latex/tables/main-mc}
\input{latex/tables/main-gen}


\subsection{Baselines}
\label{sec:setting-baseline}

A representative multilingual LLM is selected as the backbone for us to test multilingual intervention in the experiments: \bloomz\footnote{https://huggingface.co/bigscience/bloomz-7b1-mt} \citep{bloomz}. For the seven NLP tasks except \mgsm, we designate the performance of \bloomz as our standard \textbf{baseline}. For the \mgsm task, we employ the \mathllama\footnote{https://huggingface.co/Mathoctopus/Parallel\_7B} \citep{mathoctopus}, a specialized model fine-tuned for reasoning tasks, as the baseline. We compare \ours against several established techniques: (1) \textbf{\mtgoogle} Utilizing Google Translation to convert non-English questions into English, substituting the original LLM prompt. (2)\textbf{\mtllm} Leveraging \bloomz to translate queries into English, employing the structured prompt template ``\{Source Language\}: \{Inputs\} English:''. (3) \textbf{\sft} Fine-tuning all parameters of the \bloomz on an English training dataset and evaluating this on a multilingual test set. (4) \textbf{\iti} \citet{iti}Implementing an Inference-Time Intervention method by modifying the focus of attention heads within the model, adapting activation directions to shift from non-English to English. (5) \textbf{\caa}: \citet{caa} uses the difference in hidden states between non-English and English examples as a steering vector to adjust activations appropriately.

\subsection{Configuration}
\label{sec:setting-configuration}
For the training data of projection vector, we randomly sample 500 parallel items form the News Commentary dataset for each non-English and English pair. This dataset is an out-of-domain resource chosen to minimize potential biases related to the downstream tasks, focusing exclusively on intrinsic language differences.


We estimate the performance of \ours with intervening on the all layers of LLMs, using the $\alpha$ hyperparameter, which is optimized based on validation set outcomes, with values ranging from -1 to 1. We then select the optimal hyperparameter for evaluating \ours on the test set.



All experiments are conducted on a single NVIDIA A-100 GPU (40G).

==> tables/detail-patch.tex <==
\begin{table*}[h] \tiny
\centering
\begin{tabular}{lccccccccccccccc}
\toprule
\textbf{\xcopa}  & \textbf{en} & \textbf{et}  & \textbf{id}  & \textbf{it}  & \textbf{sw}  & \textbf{ta}  & \textbf{th}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}    & 76.40 & 50.80 & 69.60 & 58.60 & 55.20 & 71.60 & 50.60 & 49.60 & 71.20 & 77.40 & & & & & 61.62 \\
\textbf{patch-hidden}  &   & 76.40 & 76.40 & 76.40 & 76.40 & 76.40 & 76.40 & 76.40 & 76.40 & 76.40 & & & & & 76.40 \\
\textbf{patch-attn}     &   & 29.20 & 53.40 & 35.80 & 32.00 & 51.80 & 25.00 & 32.40 & 55.60 & 67.00 & & & & & 42.47 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}55.40\\ (+4.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}73.40\\ (+3.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}62.80\\ (+4.20)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}59.80\\ (+4.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}73.40\\ (+1.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}52.60\\ (+2.00)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}53.40\\ (+3.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}76.20\\ (+5.00)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}80.00\\ (+2.60)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}65.22\\ (+3.60)\end{tabular}} \\ \hline
\textbf{\xstorycloze}  & \textbf{en} & \textbf{ar}  & \textbf{es}  & \textbf{hi}  & \textbf{id}  & \textbf{ru}  & \textbf{sw}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}    & 91.46 & 79.22 & 87.89 & 76.37 & 84.45 & 57.78 & 50.50 & 88.55 & & & & & & & 74.96 \\
\textbf{patch-hidden}  &   & 91.46 & 91.46 & 91.46 & 91.46 & 91.46 & 91.46 & 91.46 & & & & & & & 91.46 \\
\textbf{patch-attn}     &   & 54.53 & 78.23 & 45.73 & 63.53 & 11.18 & 16.15 & 73.33 & & & & & & & 48.96 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}83.12\\ (+3.91)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}90.60\\ (+2.71)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}81.47\\ (+5.10)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}86.10\\ (+1.66)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}67.24\\ (+9.46)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}59.70\\ (+9.20)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}91.20\\ (+2.65)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}79.92\\ (+4.95)\end{tabular}} \\ \hline
\textbf{\xwinograd}    & \textbf{en} & \textbf{fr}  & \textbf{ja}  & \textbf{pt}  & \textbf{ru}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}& 73.76 & 59.04 & 51.51 & 57.80 & 54.60 & 62.30 & & & & & & & & & 57.05 \\ 
\cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}63.86\\ (+4.82)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}53.18\\ (+1.67)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}58.56\\ (+0.76)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}57.46\\ (+2.86)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}63.69\\ (+1.39)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}59.35\\  (2.30)\end{tabular}}  \\ \hline
\textbf{\xcsqa}  & \textbf{en} & \textbf{ar}  & \textbf{de}  & \textbf{es}  & \textbf{fr}  & \textbf{hi}  & \textbf{it}  & \textbf{ja}  & \textbf{nl}  & \textbf{pt}  & \textbf{ru}  & \textbf{sw}  & \textbf{vi}  & \textbf{zh}  & \textbf{AVG} \\
\textbf{baseline}    & 76.50 & 52.40 & 33.90 & 64.30 & 63.30 & 48.50 & 41.30 & 36.00 & 28.70 & 61.30 & 33.20 & 40.50 & 55.20 & 57.00 & 47.35 \\
\textbf{patch-hidden}  &   & 20.40 & 18.10 & 20.00 & 22.10 & 20.80 & 20.40 & 18.50 & 20.60 & 24.30 & 19.90 & 19.80 & 20.40 & 20.90 & 20.48 \\
\textbf{patch-attn}     &   & 46.10 & 29.90 & 58.40 & 56.80 & 40.60 & 37.60 & 32.70 & 26.40 & 57.20 & 30.10 & 36.40 & 49.50 & 50.10 & 42.45 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}53.20\\ (+0.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}34.90\\ (+1.00)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}65.00\\ (+0.70)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}63.80\\ (+0.50)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}48.80\\ (+0.30)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}42.90\\ (+1.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}36.80\\ (+0.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}29.80\\ (+1.10)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}62.60\\ (+1.30)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}33.80\\ (+0.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}42.20\\ (+1.70)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}57.30\\ (+2.10)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}58.70\\ (+1.70)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}48.45\\ (+1.09)\end{tabular}} \\ \hline
% \textbf{AmazonReview} & \textbf{en} & \textbf{de}  & \textbf{es}  & \textbf{fr}  & \textbf{ja}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
% \textbf{baseline}    & 76.32 & 71.82 & 76.25 & 76.47 & 69.88 & 68.79 & & & & & & & & & 72.64 \\ 
% \textbf{MT-Google}&     &  76.34 & 76.15 & 76.44 & 74.01 & 68.18 & & & & & & & &  & 74.22 \\
% \textbf{MT-LLM} &   &  69.64 & 75.59 & 76.01 & 68.34 & 67.48 & & & & & & & & & 71.41   \\
% \cdashline{1-16}[1pt/1pt]
% \textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}72.62\\ (+0.81)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}76.36\\ (+0.11)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}76.62\\ (+0.15)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}70.61\\ (+0.73)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}69.00\\ (+0.21)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}73.02\\ (+0.40)\end{tabular}} \\ \hline
\textbf{\xnli}   & \textbf{en} & \textbf{ar}  & \textbf{de}  & \textbf{el}  & \textbf{es}  & \textbf{fr}  & \textbf{hi}  & \textbf{ru}  & \textbf{sw}  & \textbf{th}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}    & 54.81 & 53.63 & 43.33 & 41.04 & 51.36 & 50.54 & 50.16 & 47.80 & 45.01 & 40.32 & 34.93 & 49.68 & 49.92 & & 46.48 \\
\textbf{patch-hidden}  &   & 54.81 & 54.81 & 54.81 & 54.81 & 54.81 & 54.81 & 54.79 & 54.81 & 54.81 & 54.81 & 54.81 & 54.81 & & 54.81 \\
\textbf{patch-attn}     &   & 55.95 & 50.84 & 51.88 & 56.01 & 54.87 & 54.91 & 53.39 & 53.35 & 50.74 & 50.60 & 54.89 & 55.23 & & 53.55 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}53.89\\ (+0.26)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}47.74\\ (+4.41)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}41.96\\ (+0.92)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}54.33\\ (+2.97)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}53.11\\ (+2.58)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}50.50\\ (+0.34)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}49.22\\ (+1.42)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}45.99\\ (+0.98)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}41.28\\ (+0.96)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}37.17\\ (+2.24)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.12\\ (+1.44)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.16\\ (+1.24)\end{tabular}} & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}48.12\\ (+1.65)\end{tabular}} \\ \hline
\textbf{\mzsre}  & \textbf{en} & \textbf{de}  & \textbf{es}  & \textbf{fr}  & \textbf{pt}  & \textbf{ru}  & \textbf{th}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}    & 96.23 & 55.05 & 48.86 & 49.53 & 45.49 & 30.55 & 6.33  & 38.76 & 51.68 & 33.38 & & & & & 39.96 \\
\textbf{patch-hidden}  &   & 74.83 & 75.24 & 74.16 & 73.62 & 63.66 & 45.36 & 66.89 & 73.35 & 73.89 & & & & & 69.00 \\
\textbf{patch-attn}     &   & 55.99 & 54.78 & 54.64 & 52.36 & 27.46 & 7.94  & 43.07 & 57.74 & 42.66 & & & & & 44.07 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}57.20\\ (+2.15)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}53.30\\ (+4.44)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}52.09\\ (+6.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.28\\ (+5.79)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}31.49\\ (+0.94)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}7.40\\ (+1.08)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}41.86\\ (+3.10)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}55.32\\ (+3.63)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}38.49\\ (+5.11)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}43.22\\ (+3.26)\end{tabular}} \\ \hline
\textbf{\flores} & \textbf{en} & \textbf{ar}  & \textbf{el}  & \textbf{es}  & \textbf{fr}  & \textbf{hi}  & \textbf{ru}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{AVG} \\
\textbf{baseline}    & 98.89 & 64.82 & 40.03 & 52.52 & 62.98 & 65.02 & 47.47 & 34.62 & 61.66 & 57.87 & & & & & 54.11 \\
\textbf{patch-hidden}  &   & 66.76 & 40.35 & 54.37 & 64.08 & 67.18 & 49.30 & 39.91 & 63.31 & 60.28 & & & & & 56.17 \\
\textbf{patch-attn}     &   & 64.65 & 37.26 & 52.46 & 62.56 & 64.83 & 46.43 & 33.59 & 61.88 & 57.79 & & & & & 53.49 \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}c@{}}65.61\\ (+0.79)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}40.53\\ (+0.50)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}54.62\\ (+2.10)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}64.39\\ (+1.40)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}66.26\\ (+1.23)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}48.28\\ (+0.81)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}35.91\\ (+1.29)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}63.72\\ (+2.07)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}58.71\\ (+0.84)\end{tabular}} & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{}    & \textbf{\begin{tabular}[c]{@{}c@{}}55.34\\ (+1.23)\end{tabular}} \\ \hline
\textbf{\mgsm}   & \textbf{en} & \textbf{de}   & \textbf{es}   & \textbf{fr}   & \textbf{ja}   & \textbf{ru}   & \textbf{sw}   & \textbf{th}   & \textbf{zh}   & & & & &   & \textbf{AVG}  \\
\textbf{baseline}    & 51.20 & 46.40   & 42.40   & 42.40   & 35.20   & 38.40   & 34.80   & 35.60   & 39.60   & & & & &   & 39.35   \\
\textbf{patch-hidden}  & 51.20   & 42.80  & 42.80  & 41.60  & 34.40  & 40.80  & 36.00  & 30.80  & 37.60   & & & & &   & 39.78  \\
\textbf{patch-attn}     & 51.20   & 44.00  & 44.00  & 41.20  & 37.20  & 40.40  & 36.00  & 36.40  & 37.60   & & & & &   & 40.89  \\ \cdashline{1-16}[1pt/1pt]
\textbf{\ours}&   & \textbf{\begin{tabular}[c]{@{}l@{}}48.40\\ (+2.0)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}46.80\\ (+4.4)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}45.20\\ (+2.8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}37.60\\ (+2.4)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}44.80\\ (+6.4)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}38.00\\ (+3.2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}38.80\\ (+3.2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}43.20\\ (+3.6)\end{tabular}}  & & & &  &  & \textbf{\begin{tabular}[c]{@{}l@{}}42.85\\ (+3.5)\end{tabular}}

 \\
\bottomrule
\end{tabular}
\caption{\label{tab:patch-overall} The overall results of eight NLP tasks with copying hidden states or the output of attention layer.}
\end{table*}


==> tables/details.tex <==
\begin{table*}[h] \tiny
\centering
\begin{tabular}{lllllllllllllll}
\toprule
\textbf{XCOPA}     & \textbf{et}    & \textbf{id}    & \textbf{it}    & \textbf{sw}    & \textbf{ta}    & \textbf{th}    & \textbf{tr}    & \textbf{vi}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 50.80& 69.60& 58.60& 55.20& 71.60& 50.60& 49.60& 71.20& 77.40&&&&& 61.62\\
\textbf{\ourshidden} & 51.80& 71.80& \textbf{62.80} & 59.60& 72.20& 52.00& 51.40& \textbf{76.20} & \textbf{80.00} &&&&& 64.20\\
\textbf{\oursattn}   & 52.00	 & \textbf{73.40}	 & \textbf{62.80}	 & 56.00	 & 72.80	 & 52.20	 & 51.80	 & 74.40	 & 79.40
&&&&& 63.87\\
\textbf{\oursact}   & \textbf{55.40} & 70.40& 60.80& 58.00& \textbf{73.40} & \textbf{52.60} & \textbf{53.40} & 71.80& 78.20&&&&& 63.78\\
\textbf{\oursffn}   & 53.40& 72.80 & 62.00& \textbf{59.80} & 72.40& 52.00& 52.80& 73.60& 79.20&&&&& \textbf{64.22} \\ \hline
\textbf{\xstorycloze}   & \textbf{ar}    & \textbf{es}    & \textbf{hi}    & \textbf{id}    & \textbf{ru}    & \textbf{sw}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 79.22& 87.89& 76.37& 84.45& 57.78& 50.50& 88.55&&&&&&& 74.96\\
\textbf{\ourshidden} & \textbf{83.12} & \textbf{90.60} & 78.62& 85.04& 62.01& \textbf{59.70} & \textbf{91.20} &&&&&&& \textbf{78.61} \\
\textbf{\oursattn}   & 80.15	& 89.21	& \textbf{81.47}	& 85.84	& 61.81	& 51.22	& 90.07 &&&&&&& 77.11\\
\textbf{\oursact}   & 82.46& 90.47& 78.95 & \textbf{86.10} & \textbf{63.80} & 53.01& 90.80&&&&&&& 77.94\\
\textbf{\oursffn}   & 81.73& 89.48& 78.62& 85.77& 67.24& 53.21& 91.13&&&&&&& 78.17\\ \hline
\textbf{\xwinograd} & \textbf{fr}    & \textbf{ja}    & \textbf{pt}    & \textbf{ru}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 59.04& 51.51& 57.80& 54.60& 62.30&&&&&&&&& 57.05\\
\textbf{\ourshidden} & 62.65& 52.14& 58.56& \textbf{57.46} & \textbf{63.69} &&&&&&&&& 58.90\\
\textbf{\oursattn}   & 61.45	 & 52.66	 & 58.56	 & 57.14	 & 63.29
   &&&&&&&&& 58.62\\
\textbf{\oursact}   & \textbf{63.86} & \textbf{53.18} & 58.56& 55.87& 63.49&&&&&&&&& \textbf{58.99} \\
\textbf{\oursffn}   & 60.24& 52.56& 58.18& 55.56& 63.29&&&&&&&&& 57.96\\ \hline
\textbf{\mzsre}     & \textbf{de}    & \textbf{es}    & \textbf{fr}    & \textbf{pt}    & \textbf{ru}    & \textbf{th}    & \textbf{tr}    & \textbf{vi}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 55.05& 48.86& 49.53& 45.49& 30.55& 6.33 & 38.76& 51.68& 33.38&&&&& 39.96\\
\textbf{\ourshidden} & \textbf{57.20} & \textbf{53.30} & 51.55& 51.28 & \textbf{31.49} & 7.00 & 38.76& \textbf{55.32} & 34.99&&&&& 42.32\\
\textbf{\oursattn}   & 56.66	& 52.62	& 51.82	& \textbf{52.09}	& 31.22	& 6.59	& 38.90	& 55.05	& 34.59  &&&&& 42.02\\
\textbf{\oursact}   & 56.12& 51.68& 50.07& 49.13& 31.09& 7.13 & 41.18& 52.89& 35.80&&&&& 41.68\\
\textbf{\oursffn}   & 56.80& 51.95& \textbf{51.82} & 49.93& 31.36& \textbf{7.40}  & \textbf{41.86} & 52.89& \textbf{38.49} &&&&& \textbf{42.50} \\ \hline
\textbf{\flores}    & \textbf{ar}    & \textbf{el}    & \textbf{es}    & \textbf{fr}    & \textbf{hi}    & \textbf{ru}    & \textbf{tr}    & \textbf{vi}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 64.82& 40.03& 52.52& 62.98& 65.02& 47.47& 34.62& 61.66& 57.87&&&&& 54.11\\
\textbf{\ourshidden} & \textbf{65.61} & 39.79& \textbf{54.62} & \textbf{64.39} & 65.56& 47.93& 34.67& 62.88& \textbf{58.71} &&&&& 54.91\\
\textbf{\oursattn}   & 65.57& 40.28& 54.39& 64.24& 65.28& \textbf{48.28} & \textbf{35.91} & 62.69& 58.59&&&&& 55.03\\
\textbf{\oursact}   & 65.61& 40.25& 54.61& 64.37& \textbf{66.26} & 47.54& 34.81& \textbf{63.72} & 58.70&&&&& \textbf{55.10} \\
\textbf{\oursffn}   & 64.95& \textbf{40.53} & 52.82& 63.20& 65.69& 47.85& 34.83& 61.91& 58.39&&&&& 54.46\\ \hline
\textbf{\xcsqa}     & \textbf{ar}    & \textbf{de}    & \textbf{es}    & \textbf{fr}    & \textbf{hi}    & \textbf{it}    & \textbf{ja}    & \textbf{nl}    & \textbf{pt}    & \textbf{ru}    & \textbf{sw}    & \textbf{vi}    & \textbf{zh}    & \textbf{AVG}   \\
\textbf{\baseline} & 52.40& 33.90& 64.30& 63.30& 48.50& 41.30& 36.00& 28.70& 61.30& 33.20& 40.50& 55.20& 57.00& 47.35\\
\textbf{\ourshidden} & 52.60& 34.60 & \textbf{65.00} & \textbf{63.80} & 48.40& \textbf{42.90} & 36.70& 29.00& \textbf{62.60} & 33.50& 41.60& 57.00 & \textbf{58.70} & 48.18 \\
\textbf{\oursattn}   & \textbf{53.20}	& \textbf{34.90}	& 64.80	& 63.60	& \textbf{48.80}	& 41.90	& \textbf{36.80}	& 28.80	& 62.20	& \textbf{33.80}	& \textbf{42.20}	& \textbf{57.30}	& 58.30	& \textbf{48.20}
\\
\textbf{\oursact}   & 52.70& 33.80& 64.50& 63.40& 48.30& 42.20& 36.70& 29.80& 61.60& 33.30& 41.20& 55.60& 57.90& 47.77\\
\textbf{\oursffn}   & 52.80& 33.80& 64.80& 63.40& 48.60& 42.50& \textbf{36.80} & \textbf{29.60} & 62.10& 33.70 & 42.00 & 55.70& 57.70& 47.96\\ \hline
% \textbf{Amazon Review} & \textbf{de}    & \textbf{es}    & \textbf{fr}    & \textbf{ja}    & \textbf{zh}    & \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{}& \textbf{AVG}   \\
% \textbf{\baseline} & 71.82& 76.25& 76.47& 69.88& 68.79&&&&&&&&& 72.64\\
% \textbf{\ourshidden} & \textbf{72.73} & \textbf{76.34 }   & 76.51& \textbf{70.65} & 68.90&&&&&&&&& \textbf{73.02} \\
% \textbf{\oursattn}   & 72.62	 & 76.34	 & 76.51	 & 70.61	 & \textbf{69.00}
% &&&&&&&&& 73.02\\
% \textbf{\oursact}   & 71.98& 76.34& 76.51& 70.18& 68.90&&&&&&&&& 72.78\\
% \textbf{\oursffn}   & 72.60& 76.36& \textbf{76.62} & 70.31& 68.94 &&&&&&&&& 72.97\\ \hline
\textbf{\xnli}& \textbf{ar}    & \textbf{de}    & \textbf{el}    & \textbf{es}    & \textbf{fr}    & \textbf{hi}    & \textbf{ru}    & \textbf{sw}    & \textbf{th}    & \textbf{tr}    & \textbf{vi}    & \textbf{zh}    & \textbf{}& \textbf{AVG}   \\
\textbf{\baseline} & 53.63& 43.33& 41.04& 51.36& 50.54& 50.16& 47.80& 45.01& 40.32& 34.93& 49.68& 49.92&& 46.48\\
\textbf{\ourshidden} & 53.83& 47.21 & \textbf{41.96} & 52.77& 52.26& \textbf{50.44} & 48.72& 45.47& 40.50& 35.17& 50.48& \textbf{51.16} && 47.50\\
\textbf{\oursattn}   & 53.83	& \textbf{47.74}	& 41.34	& 53.79  & 	52.95	& 50.44	& \textbf{49.22}	& \textbf{45.99}	& \textbf{41.28}	& \textbf{37.17}	& \textbf{51.12}	& 50.12
    && \textbf{47.92} \\
\textbf{\oursact}   & 53.73& 45.21& 41.54& \textbf{54.33 }   & \textbf{53.11  }  & 50.28& 49.02& 45.31& 40.76& 36.45& 51.12& 50.74&& 47.63\\
\textbf{\oursffn}   & \textbf{53.89} & 45.17& 41.18& 52.97& 53.01& 50.50& 49.06 & 45.69& 40.50& 36.87 & 50.58& 50.20&& 47.47 \\
\bottomrule
\end{tabular}
\caption{\label{tab:detail} The results of intervention in the hidden states, output of attention layer, output of the first FFN layer, output of the second FFN layer.}
\end{table*}

==> tables/fewshots.tex <==
\begin{table*}[h] \scriptsize
\centering
\begin{tabular}{lcccccccccc}
\toprule
& \textbf{de}  & \textbf{es}  & \textbf{fr}  & \textbf{pt}  & \textbf{ru}  & \textbf{th} & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{AVG} \\ \hline
\textbf{0-shot \baseline} & 55.05  & 48.86  & 49.53  & 45.49  & 30.55  & 6.33  & 38.76  & 51.68  & 33.38  & 39.96  \\
0-shot \ours& \textbf{\begin{tabular}[c]{@{}c@{}}57.20\\ (+2.15)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}53.30\\ (+4.44)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.55\\ (+2.02)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.28\\ (+5.79)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}31.49\\ (+0.94)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}7.00\\ (+0.67)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}38.76\\ (+0.00)\end{tabular}& \textbf{\begin{tabular}[c]{@{}c@{}}55.32\\ (+3.63)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}34.99\\ (+1.62)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}42.32\\ (+2.36)\end{tabular}} \\ \hline
\textbf{2-shot \baseline} & 65.41  & 57.47  &56.26	&57.34 &34.18	&9.56	&50.47	&58.41	&41.32		&47.82  \\
2-shot \ours& \begin{tabular}[c]{@{}c@{}}65.41\\ (+0.00)\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}58.01\\ (+0.54)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}57.87\\ (+1.62)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}60.03\\ (+2.69)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}34.99\\ (+0.81)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}9.83\\ (+0.27)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}51.01\\ (+0.54)\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}60.97\\ (+2.56)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}43.74\\ (+2.42)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}49.10\\ (+1.27)\end{tabular}} \\ \hline
\textbf{4-shot \baseline} & 71.06  & 64.33  & 62.72  & 66.22  & 42.53  & 13.19 & 55.72  & 67.03  & 51.95  & 54.97  \\
4-shot \ours& \textbf{\begin{tabular}[c]{@{}c@{}}71.60\\ (+0.54)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}67.56\\ (+3.23)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}64.06\\ (+1.35)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}67.29\\ (+1.08)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}42.66\\ (+0.13)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}13.19\\ (+0.00)\end{tabular}   & \textbf{\begin{tabular}[c]{@{}c@{}}56.26\\ (+0.54)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}68.78\\ (+1.75)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}52.49\\ (+0.54)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}55.99\\ (+1.02)\end{tabular}} \\
\bottomrule
\end{tabular}
\caption{\label{tab:few-shots} The comparison of \mzsre dataset with \ours based on the zero-shot setting and few-shot setting.}
\end{table*}

==> tables/multilingual_prompt.tex <==
\begin{table*}[]\scriptsize
\centering
\begin{tabular}{lccccccccccc}
\toprule
&  & \textbf{et}   & \textbf{id}   & \textbf{it}   & \textbf{sw}   & \textbf{ta}& \textbf{th}   & \textbf{tr}& \textbf{vi}   & \textbf{zh}  & \textbf{AVG}\\ \hline
\multirow{2}{*}{\textbf{English template}}     & \textbf{baseline} & 50.80    & 69.60& 58.60& 55.20& 71.60& 50.60& 49.60 & 71.20& 77.40     & 61.62\\
& \textbf{\ours}& \textbf{\begin{tabular}[c]{@{}c@{}}51.80\\ (+1.00)\end{tabular}}     & \textbf{\begin{tabular}[c]{@{}c@{}}71.80\\ (+2.20)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}62.80\\ (+4.20)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}59.60   \\ (+4.4)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}72.20   \\ (+0.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}52.00\\ (+1.40)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}51.40 \\ (+1.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}76.20\\ (+5.0)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}80.00\\ (+2.65)\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}64.20\\ (+2.58)\end{tabular}}  \\ \hline
\multirow{2}{*}{\textbf{multilingual template}} & \textbf{baseline} & 49.20   & 65.60& 55.00& 56.20& 63.00& 50.40& 49.20 & 69.40& 73.80     & 59.09\\
& \textbf{\ours}& \textbf{\begin{tabular}[c]{@{}c@{}}51.80  \\ (+2.60)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}69.00  \\ (+3.40)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}56.00  \\ (+1.00)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}57.00  \\ (+0.80)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}64.40\\ (+1.40)\end{tabular}}    & \begin{tabular}[c]{@{}c@{}}50.20\\ (-0.20)\end{tabular}   & \textbf{\begin{tabular}[c]{@{}c@{}}54.2   \\ (+5.0)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}70.40  \\ (+1.00)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}77.40 \\ (+3.60)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}61.16  \\ (+2.07)\end{tabular}} \\
\bottomrule
\end{tabular}
\caption{\label{tab:non-english prompt} The results of \xcopa dataset with \ours under the English prompt template with the multilingual prompt template.}
\end{table*}

==> tables/patching.tex <==
\begin{table*}[h]\small
\centering
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{11}{c}{multiple-choice task} \\ \midrule   
\textbf{\xcopa}             & \textbf{et}  & \textbf{id}  & \textbf{it}  & \textbf{sw}  & \textbf{ta}  & \textbf{th}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{AVG} \\
% \textbf{baseline}       & 76.40& 50.80        & 69.60        & 58.60        & 55.20        & 71.60        & 50.60        & 49.60        & 71.20        & 77.40        & 61.62        \\
\textbf{\textsc{patch-hidden}}   & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & \textbf{76.40}     & 76.40        & \textbf{76.40}     \\
\textbf{\textsc{patch-attn}}     & 29.20        & 53.40        & 35.80        & 32.00        & 51.80        & 25.00        & 32.40        & 55.60        & 67.00        & 42.47        \\
\textbf{\ourshidden}  & \multicolumn{1}{l}{51.80}          & \multicolumn{1}{l}{71.80}          & \multicolumn{1}{l}{62.80}          & \multicolumn{1}{l}{59.60}          & \multicolumn{1}{l}{72.20}          & \multicolumn{1}{l}{52.00}          & \multicolumn{1}{l}{51.40}          & \multicolumn{1}{l}{76.20}          & \multicolumn{1}{l}{\textbf{80.00}}          & \multicolumn{1}{l}{64.20}          \\
\textbf{\oursattn}    & \multicolumn{1}{l}{52.00}          & \multicolumn{1}{l}{73.40}          & \multicolumn{1}{l}{62.80}          & \multicolumn{1}{l}{56.00}          & \multicolumn{1}{l}{72.80}          & \multicolumn{1}{l}{52.20}          & \multicolumn{1}{l}{51.80}          & \multicolumn{1}{l}{74.40}          & \multicolumn{1}{l}{79.40} & \multicolumn{1}{l}{63.87}          \\ \midrule
\multicolumn{11}{c}{open-ended generation task (output in English)} \\ \midrule 
\textbf{\flores}          & \textbf{ar}  & \textbf{el}  & \textbf{es}  & \textbf{fr}  & \textbf{hi}  & \textbf{ru}  & \textbf{tr}  & \textbf{vi}  & \textbf{zh}  & \textbf{AVG} \\
% \textbf{baseline}       & -    & 64.82        & 40.03        & 52.52        & 62.98        & 65.02        & 47.47        & 34.62        & 61.66        & 57.87        & 54.11        \\
\textbf{\textsc{patch-hidden}}   & \textbf{66.76}     & \textbf{40.35}     & 54.37        & 64.08        & \textbf{67.18}     & \textbf{49.30}     & \textbf{39.91}     & \textbf{63.31}     & \textbf{60.28}     & \textbf{56.17}     \\
\textbf{\textsc{patch-attn}}     & 64.65        & 37.26        & 52.46        & 62.56        & 64.83        & 46.43        & 33.59        & 61.88        & 57.79        & 53.49        \\
\textbf{\ourshidden}& \multicolumn{1}{l}{65.61}          & \multicolumn{1}{l}{39.79}          & \multicolumn{1}{l}{\textbf{54.62}} & \multicolumn{1}{l}{\textbf{64.39}}          & \multicolumn{1}{l}{65.56}          & \multicolumn{1}{l}{47.93}          & \multicolumn{1}{l}{34.67}          & \multicolumn{1}{l}{62.88}          & \multicolumn{1}{l}{58.71}          & \multicolumn{1}{l}{54.91}          \\
\textbf{\oursattn}    & \multicolumn{1}{l}{65.57}          & \multicolumn{1}{l}{40.28}          & \multicolumn{1}{l}{54.39}          & \multicolumn{1}{l}{64.24} & \multicolumn{1}{l}{65.28}          & \multicolumn{1}{l}{48.28}          & \multicolumn{1}{l}{35.91}          & \multicolumn{1}{l}{62.69}          & \multicolumn{1}{l}{58.59}          & \multicolumn{1}{l}{55.03}          \\ \midrule
\multicolumn{11}{c}{open-ended generation task (output in non-English)} \\ \midrule 
\textbf{\mgsm}        & \textbf{de}  & \textbf{es}  & \textbf{fr}  & \textbf{ja}  & \textbf{ru}  & \textbf{sw}  & \textbf{th}  & \textbf{zh}  &              & \textbf{AVG} \\
% \textbf{baseline}     & 46.40        & 42.40        & 42.40        & 35.20        & 38.40        & 34.80        & 35.60        & 39.60        &              & 39.35        \\
\textbf{\textsc{patch-hidden}}   & 42.80        & 42.80        & 41.60        & 34.40        & 40.80        & 36.00        & 30.80        & 37.60        &              & 39.78        \\
\textbf{\textsc{patch-attn}}     & 44.00        & 44.00        & 41.20        & 37.20        & 40.40        & 36.00        & 36.40        & 37.60        &              & 40.89        \\
\textbf{\ourshidden}  & \multicolumn{1}{l}{\textbf{47.60}} & \multicolumn{1}{l}{\textbf{46.80}} & \multicolumn{1}{l}{\textbf{44.40}} & \multicolumn{1}{l}{36.00}          & \multicolumn{1}{l}{\textbf{44.40}} & \multicolumn{1}{l}{\textbf{38.00}} & \multicolumn{1}{l}{37.60}          & \multicolumn{1}{l}{\textbf{43.20}} & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{\textbf{42.25}} \\
\textbf{\oursattn}   & \multicolumn{1}{l}{\textbf{47.60}} & \multicolumn{1}{l}{45.20}          & \multicolumn{1}{l}{44.00}          & \multicolumn{1}{l}{\textbf{37.60}} & \multicolumn{1}{l}{42.00}          & \multicolumn{1}{l}{36.80}          & \multicolumn{1}{l}{\textbf{38.80}} & \multicolumn{1}{l}{40.40}          & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{41.55}         \\
\bottomrule
\end{tabular}
\caption{\label{tab:patch} Comparison between patching representations and \ours.}
\end{table*}


==> tables/time.tex <==
% \begin{table}[h] \small
% \centering
% \begin{tabular}{lcc}
% \toprule
%  & Multiple Choice    & Open-ended Generation   \\ \hline
% \baseline & 0.11s & 0.71s \\
% \opurs  & 0.20s & 0.80s \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:infer-time} Time consuming of \baseline and \ours  on the \copa (multiple choice task) and \flores (open-ended generation) dataset with \bloomz.}
% \end{table}

\begin{table}[h] \small
\centering
\begin{tabular}{lc}
\toprule
infer time &  1 item  \\ \hline
\baseline  & 0.71s \\
\ours  & 0.80s \\
\bottomrule
\end{tabular}
\caption{\label{tab:infer-time} Time consuming of \baseline and \ours  on the \flores dataset with \bloomz.}
\end{table}
